Determinant-Preserving Sparsification of SDDM Matrices with Applications to Counting and Sampling Spanning Trees

We show variants of spectral sparsification routines can preserve the total spanning tree counts of graphs, which by Kirchhoff's matrix-tree theorem, is equivalent to determinant of a graph Laplacian minor, or equivalently, of any SDDM matrix. Our analyses utilizes this combinatorial connection to bridge between statistical leverage scores / effective resistances and the analysis of random graphs by [Janson, Combinatorics, Probability and Computing `94]. This leads to a routine that in quadratic time, sparsifies a graph down to about $n^{1.5}$ edges in ways that preserve both the determinant and the distribution of spanning trees (provided the sparsified graph is viewed as a random object). Extending this algorithm to work with Schur complements and approximate Choleksy factorizations leads to algorithms for counting and sampling spanning trees which are nearly optimal for dense graphs. We give an algorithm that computes a $(1 \pm \delta)$ approximation to the determinant of any SDDM matrix with constant probability in about $n^2 \delta^{-2}$ time. This is the first routine for graphs that outperforms general-purpose routines for computing determinants of arbitrary matrices. We also give an algorithm that generates in about $n^2 \delta^{-2}$ time a spanning tree of a weighted undirected graph from a distribution with total variation distance of $\delta$ from the $w$-uniform distribution .

==> spanning_tree_level.tex <==
\subsection{Total Variation Distance Between Distributions
	Produced by Layer-Truncated Algorithms}
\label{subsec:TVPerLayer}
	
	



For this, we need to consider `split sequences', which represent
the possible ways of partitioning into $V_1 \sqcup V_2$,
as well as ways of contracting edges contained in $V_1$.
\begin{definition}
	\label{def:splitSq}
	We use $\mathcal{S}^{l}$ to denote the space of possible split
	sequences made by recursive calls between levels $0$ and $l - 1$.
	Such a sequence specifies the number of graphs on level $l$,
	as well as the vertices passed to them.
	
	Given a split sequence $S \in \mathcal{S}^{l}$, we use
	$\Pr^{\textsc{AIS}}(S)$ (abbreviation for almost independent set)
	to denote the probability of the $V_1$s being picked over the space
	of all the calls.
	
	Furthermore, we use $k_{S}$ to denote the number of graphs on
	level $l$ of this split sequence, and
	$\vec{\mathcal{G}}(S)$ to denote the distribution over graphs on
	these $k_{S}$ vertex sets specified by $S$,
	$G^{S}_1 \ldots G^{S}_{k_S}$, which we also denote
	as $\vec{G}^{S}$.
\end{definition}

The probability of a particular tree $\hatT$ being produced
is then given by:
\begin{lemma}
	\label{lem:lol}
	For a particular tree $\hatT$, we can create a list of combinatorial
	trees, one per split sequence $S$, $\vec{\mathcal{T}}(S, \hatT)$,
	along with an associated probability of each of tree sequences
	being mapped back to $\hatT$ via the various prolongation calls:
	\[
	p^{\uparrow}(S, \vec{G}^{S}, \hatT, \vec{T})
	\]
	such that:
	\[
	\Pr^{\mathcal{T}^{l}}\left(\hatT \right)
	= \sum_{S \in \mathcal{S}^{l}}
	\Pr^{AIS}\left(S\right)
	\cdot
	\expec{\vec{G}^{S} \in \vec{\mathcal{G}} \left(S\right)}
	{\sum_{ \vec{T}^{S} \in \vec{\mathcal{T}}\left( S, \hatT \right)}
		p^{\uparrow}\left(S, \vec{G}^{S}, \hatT, \vec{T}\right) \cdot 
		\prod_{j = 1}^{k_{S}} \Pr^{G^{S}_j}\left(\vec{T}^{S}_j \right)},
	\]
	and by letting the distribution produced by
	$\textsc{IdealSparsify}(G^{S}_j, |V(G^{S}_j) |/ \overline{n})$ be
	$\mathcal{H}^{S}_j$, we get
	\[
	\Pr^{\mathcal{T}^{l + 1}}\left(\hatT \right)
	= \sum_{S \in \mathcal{S}^{l}}
	\Pr^{\textsc{AIS}}\left(S\right)
	\expec{\vec{G}^{S} \in \vec{\mathcal{G}}\left(S\right)}
	{\sum_{ \vec{T}^{S}
			\in \vec{\mathcal{T}}\left( S, \hatT \right)}
		p^{\uparrow}\left(S, \vec{G}^{S}, \hatT, \vec{T}\right) \cdot 
		\prod_{j = 1}^{k_{S}}
		\expec{H^{S}_j \sim \mathcal{H}^{G^{S}}_{j}}
		{\Pr^{H^{S}_j}\left(\vec{T}^{S}_j \right)}}.
	\]
\end{lemma}


\todo{Define the probability of a sequence of graph
	producing a sequence of trees, $\Pr^{\vec{G}^{S}}(\vec{T}^{S})$,
	and maybe use it here?!?!}

The variance accumulation per layer can still be bounded
using the fact that for any $\vec{G}^{S}$,
\[
\sum_{i} \abs{V\left(\vec{G}^{S} \right)}
= O\left(\overline{n} \right).
\]
\begin{lemma}
	\label{lem:AccumulationVariance}
	For any $S$,
	any graph sequence $\vec{G}^{S}$,
	with associated sparsifier distribution $\mathcal{H}^{S}$,
	any tree $\hat{T}$
	and $\vec{T}^{S} \in \mathcal{T}(S, \hat{T})$ such
	that $\Pr^{\vec{G}^{S}}(\vec{T}^{S}) > 0$, we have
	\[
	\prob{\vec{H}^{S} \sim \vec{\mathcal{H}}^{\vec{G}^S}}
	{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0}^{-1}
	\cdot 
	\expec{\vec{H}^{S} \sim \mathcal{H}^{\vec{G}^{S}}
		\left| \Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0\right.}
	{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right)^{-1}}
	= \left(1 \pm \delta \right)
	\Pr^{\vec{G}^{S}}\left(\vec{T}^{S} \right)^{-1},
	\]
	and
	\[
	\prob{\vec{H}^{S} \sim \vec{\mathcal{H}}^{\vec{G}^S}}
	{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0}^{-2}
	\cdot 
	\expec{\vec{H}^{S} \sim \mathcal{H}^{\vec{G}^{S}}
		\left| \Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0\right.}
	{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right)^{-2}}
	\leq \left(1 + \delta \right)
	\Pr^{\vec{G}^{S}}\left(\vec{T}^{S} \right)^{-2}.
	\]
	\rp{I'm making up notation as I go, fix this on next pass?!?!}
\end{lemma}
\todo{Can this talk with Lemma~\ref{lem:invVarTVBound}?!?!}
\rp{Note that the outer stuff is not a distribution over
	distributions anymore}

We can then bound the TV distance between $\mathcal{T}^{l}$
and $\mathcal{T}^{l + 1}$.

\begin{proof}(of Lemma~\ref{lem:DistPerLayer})
	
	The main idea is to bound
	\begin{multline}
	\sum_{\hatT}
	\sum_{S \in \mathcal{S}}
	\sum_{\vec{G}^{S} \in \vec{\mathcal{G}}\left(S\right)}
	\Pr^{\vec{\mathcal{G}}\left(S\right)}\left( \vec{G}^{S}  \right)
	\cdot
	\sum_{\vec{T}^{S} \in \vec{\mathcal{T}}\left(S, \hatT\right)}
	p^{\uparrow}\left(S, \vec{G}^{S}, \hatT, \vec{T}\right)
	\cdot \sum_{\vec{H}^{S} \in \mathcal{H}^{G^{S}}:
		\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0}
	\Pr^{\mathcal{H}^{G^{S}}}\left(\vec{H}^{S}\right)\\
	\cdot \Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) \cdot
	\left(
	\frac{\Pr^{\vec{G}^{S}}\left(\vec{T}^{S}\right)}
	{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S}\right)
		\cdot \prob{\vec{H}^{S} \sim \vec{\mathcal{H}}^{\vec{G}^S}}
		{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0}}
	- 1 \right)^2,
	\label{eq:SqDif}
	\end{multline}
	and then bring this to a bound that's more than
	the total variation distance via the Cauchy-Schwarz
	inequality.
	
	Note that this summation is well defined because
	the last summation requires $\Pr^{\vec{H}^{S}}(\vec{T}^{S}) > 0$,
	which in turn implies $\Pr^{\vec{G}^{S}}(\vec{T}^{S} ) > 0$
	as each graph $\vec{H}^{S}_j$ is a weighted subgraph of
	the corresponding $\vec{G}^{S}_j$.
	
	For simplicity of notation, we will use a single weight term to
	denote the product of the probability of picking $G^{S}$
	and prologating $\vec{T}^{S}$ back to $\hatT$:
	\[
	\hat{p}\left(\hatT, S, \vec{G}, \vec{T}^{S}\right)
	\defeq
	\Pr^{\vec{\mathcal{G}}\left(S\right)}\left( \vec{G}^{S}  \right)
	\cdot
	\sum_{\vec{T}^{S} \in \vec{\mathcal{T}}\left(S, \hatT\right)}
	p^{\uparrow}\left(S, \vec{G}^{S}, \hatT, \vec{T}\right),
	\]
	and abbreviate the first four summations
	we will write the first four summations
	over $\hatT$, $\S$, $\vec{G}^{S}$, $\vec{T}^{S}$ as summing
	over the choices with non-zero values of
	$\hat{p}(\hatT, S, \vec{G}, \vec{T}^{S})$.
	
	As the given conditions are a mixture of expectations
	and summations, we will only use summations in our
	notations.
	Then the two conditions provided in Lemma~\ref{lem:AccumulationVariance}
	imply that for any $\vec{G}^{S}$ and $\vec{T}^{S}$
	with $\Pr^{\vec{G}}(\vec{T}^{S}) > 0$, we have
	\[
	\sum_{\vec{H}^{S} \in \mathcal{H}^{G^{S}}:
		\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0}
	\Pr^{\mathcal{H}^{G^{S}}}\left(\vec{H}^{S}\right)
	\cdot
	\frac{\Pr^{\vec{G}^{S}}\left(\vec{T}^{S}\right)^2}
	{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S}\right)^2
		\cdot \prob{\vec{H}^{S} \sim \vec{\mathcal{H}}^{\vec{G}^S}}
		{\Pr^{\vec{H}^{S}}\left(\vec{T}^{S} \right) > 0}^2}
	\leq 1 + \delta.
	\]
	
	\todo{The hard part is that we need to somehow move the
		$\hatT$ summation into the inside, as otherwise we'd
		be proving point-wise probabilities, which cannot be true.}
	
\end{proof}




%%
%%\begin{proof}(Of Lemma\ref{lem:DistPerLayer})
%%	Because all recursive calls used to generate $\mathcal{T}^{(l)}$
%%	switch over to the un-sparsified algorithm after layer $l$,
%%	the independence claim from Claim~\ref{claim:independent} means that if we
%%	treat the set of all possible sparsifiers produced as an event $\mathcal{I}$
%%	such that each event $i \in \mathcal{I}$ produces a set of graphs
%%	correpsonding to the exact Schur complements passed to the next recursive level:
%%	\[
%%	G^{i}_1 \ldots G^{i}_{k_i}
%%	\]
%%	whose total number of vertices is $O(n)$, along with associated trees
%%	\[
%%	\hatT^{i}_1 \ldots \hatT^{i}_{k_i}
%%	\]
%%	\todo{not unique set of trees from each $G_{1}^{i}$}
%%	along with a scalar $c(i)$ such that
%%	\[
%%	\Pr^{\mathcal{T}^{\left(l \right)}}\left( \hatT \right)
%%	= \expec{i \in I}{ c\left( i \right) \cdot \prod_{j = 1}^{k_i}
%%		\Pr^{G^{i}_j}\left( \hatT^{i}_j \right) }.
%%	\]
%%	
%%	The creation of sparsifiers creates a collection of graphs,
%%	one per $G^{i}_{j}$, $\mathcal{H}^{i}_{j}$ such that
%%	\[
%%	\Pr^{\mathcal{T}^{\left(l + 1 \right)}}\left( \hatT \right)
%%	= \expec{i \in I}{ c\left( i \right) \cdot \prod_{j = 1}^{k_i}
%%		\expec{H^{i}_{j} \in \mathcal{H}^{i}_j}{\Pr^{H^{i}_{j}}\left( \hatT^{i}_j \right) }},
%%	\]
%%	and by Lemma~\ref{lem:InvConc}, for each of these $\mathcal{H}^{i}_j$
%%	we have:
%%	\begin{align*}
%%		\prob{H \sim \mathcal{H}^{i}_{j}}{\hatT^{i}_{j} \subseteq H}^{-1} \cdot 
%%		\expec{H|_{\hatT}
%%			\sim \left(\mathcal{H}^{i}_{j}\right)_{|_{\hatT^{i}_{j}}}}{
%%			\Pr^{H|_{\hatT}}\left(\hatT^{i}_{j} \right)^{-1}}
%%		& = \left(1 \pm O\left(\frac{\abs{V\left( G^{i}_{j} \right)}}{\amount}\right)\right)
%%		\Pr^{G^{i}_{j}}\left(\hatT^{i}_{j} \right)^{-1},\\
%%		\prob{H \sim \mathcal{H}}{\hatT^{i}_{j} \subseteq H}^{-2} \cdot 
%%		\var{H|_{\hatT}
%%			\sim \left(\mathcal{H}^{i}_{j}\right)_{|_{\hatT^{i}_{j}}}}{
%%			\Pr^{H|_{\hatT}}\left(\hatT^{i}_{j} \right)^{-1}}
%%		& \leq O\left(\frac{\abs{V\left( G^{i}_{j} \right)}^2}{\amount}\right)
%%		\Pr^{G^{i}_{j}}\left(\hatT^{i}_{j} \right)^{-2}.
%%	\end{align*}
%%	Plugging in the fact that on each recursive call,
%%	$s$ was set to $\delta \overline{n} \abs{V\left( G^{i}_{j} \right)}$
%%	\todo{Modify pseudocode, point to line}, these products become bounded by:
%%	\begin{align*}
%%		\prod_{j = 1}^{i_k}
%%		\prob{H \sim \mathcal{H}^{i}_{j}}{\hatT^{i}_{j} \subseteq H}^{-1} \cdot 
%%		\expec{H|_{\hatT}
%%			\sim \left(\mathcal{H}^{i}_{j}\right)_{|_{\hatT^{i}_{j}}}}{
%%			\Pr^{H|_{\hatT}}\left(\hatT^{i}_{j} \right)^{-1}}
%%		& = \left(1 \pm \delta \right)
%%		\prod_{j = 1}^{k_i} \Pr^{G^{i}_{j}}\left(\hatT^{i}_{j} \right)^{-1},\\
%%		\prod_{j = 1}^{i_k}
%%		\prob{H \sim \mathcal{H}}{\hatT^{i}_{j} \subseteq H}^{-2} \cdot 
%%		\var{H|_{\hatT}
%%			\sim \left(\mathcal{H}^{i}_{j}\right)_{|_{\hatT^{i}_{j}}}}{
%%			\Pr^{H|_{\hatT}}\left(\hatT^{i}_{j} \right)^{-1}}
%%		& \leq O\left(\delta\right)
%%		\prod_{j = 1}^{i_k}
%%		\Pr^{G^{i}_{j}}\left(\hatT^{i}_{j} \right)^{-2}.
%%	\end{align*}
%%	So we can define a new event space for the situation where we do
%%	invoke $\textsc{IdealSparsify}$ on level $l$ by considering the event
%%	\[
%%	\left( i, H^{i}_1, H^{i}_2, \ldots H^{i}_{k_i} \right).
%%	\]
%%	This event space meets the requirement of Lemma~\ref{lem:invVarTVBound},
%%	and therefore we obtain the bound on the TV distance
%%	between $\mathcal{T}^{(l)}$ and $\mathcal{T}^{(l + 1)}$.
%%\end{proof}


